Human Perception-Optimized Planning for Comfortable VR-Based Telepresence

This paper introduces an emerging motion planning problem by considering a human that is immersed into the viewing perspective of a remote robot. The challenge is to make the experience both effective (such as delivering a sense of presence) and comfortable (such as avoiding adverse sickness symptoms, including nausea). We refer to this challenging new area as human perception-optimized planning and propose a general multiobjective optimization framework that can be instantiated in many envisioned scenarios. We then consider a specific VR telepresence task as a case of human perception-optimized planning, in which we simulate a robot that sends 360 video to a remote user to be viewed through a head-mounted display. In this particular task, we plan trajectories that minimize VR sickness (and thereby maximize comfort). An A* type method is used to create a Pareto-optimal collection of piecewise linear trajectories while taking into account criteria that improve comfort. We conducted a study with human subjects touring a virtual museum, in which paths computed by our algorithm are compared against a reference RRT-based trajectory. Generally, users suffered less from VR sickness and preferred the paths created by the presented algorithm.

==> Comfortable telepresence def Rev 1/acronyms.tex <==
\newacro{vr}[VR]{Virtual Reality}
\newacro{hmd}[HMD]{Head-Mounted Display}
\newacro{ems}[EMS]{Electrical Muscle Stimulation}
\newacro{imu}[IMU]{Inertial Measurement Unit}
\newacro{bci}[BCI]{Brain-Computer Interface}
\newacro{vwg}[VWG]{Virtual World Generator}
\newacro{moo}[MOO]{Multi-Objective Optimization}
\newacro{dof}[DoF]{Degree of Freedom}
\newacro{ssq}[SSQ]{Simulator Sickness Questionnaire}

==> Comfortable telepresence def Rev 1/defs.tex <==


%% Use this to make index entries appear in the margin
%\usepackage{showidx}

%\usepackage[dvips,ps2pdf]{hyperref} 
%\usepackage{hyperref} 




%% Turn on/off math bold
\def\mbon{\mathversion{bold}}
\def\mboff{\mathversion{normal}}

%% Continuous-time definitions
\def\tf{{\phi}} %% State transition function

\def\queue{{Q}}

%% Nature actions
\def\nata{{\theta}}
\def\natas{{\Theta}} % All nature actions

\def\Xappr{{\hat{X}}} % Approximate state space
\def\Xfappr{{\tilde{X}}} % Approximate state space

%% Borrowed from Devin Balkcom and Matt Mason (ijrr 02 paper):
\newcommand{\FF}[0]{\ensuremath{\Uparrow}}
\newcommand{\BB}[0]{\ensuremath{\Downarrow}}
\newcommand{\LL}[0]{\ensuremath{\curvearrowleft}}
\newcommand{\RR}[0]{\ensuremath{\curvearrowright}}

\def\graph{{\cal G}}

\def\stages{{\cal K}}

\def\histy{{\tilde{y}}} %% History
\def\histu{{\tilde{u}}} %% History
\def\histv{{\tilde{v}}} %% History
\def\histx{{\tilde{x}}} %% History
\def\histz{{\tilde{z}}} %% History
\def\histp{{\tilde{p}}} %% History
\def\histe{{\tilde{e}}} %% History
\def\histtheta{{\tilde{\theta}}} %% History
\def\histyt{{\tilde{y}_t}} %% History
\def\histut{{\tilde{u}_t}} %% History
\def\histxt{{\tilde{x}_t}} %% History
\def\histthetat{{\tilde{\theta}_t}} %% History
\def\histpsit{{\tilde{\psi}_t}} %% History
\def\hspacey{{\tilde{Y}}} %% History
\def\hspaceu{{\tilde{U}}} %% History
\def\hspacex{{\tilde{X}}} %% History
\def\histpt{{\tilde{p}_t}} %% History
\def\histist{{\tilde \ist}}
\def\histq{{\tilde q}}
\def\histplan{{\tilde\plan}}

%% Information space notation
\def\ic{{\eta_0}} %% Initial condition
\def\ics{{{\cal I}_0}} %% Initial condition space
\def\ici{{\eta^i_0}} %% Initial condition
\def\icsi{{{\cal I}^i_0}} %% Initial condition space
\def\ist{{\eta}} %% Information state
\def\istder{{\eta_{der}}} %% Information state
\def\ifs{{\cal I}} %% An information space
\def\ifsder{{\cal I}_{der}} %% History information space
\def\ifsderp{{\cal I}'_{der}} %% History information space
\def\ifsest{{\cal I}_{est}} %% History information space
\def\ifshist{{\cal I}_{hist}} %% History information space
\def\ifsndet{{\cal I}_{ndet}} %% Nondeterministic information space
\def\ifsprob{{\cal I}_{prob}} %% Probabilistic information space
\def\ifsgauss{{\cal I}_{gauss}} %% Probabilistic information space
\def\ifsapp{{\cal I}_{app}} %% Probabilistic information space
\def\ifsmom{{\cal I}_{mom}} %% Probabilistic information space
\def\ifsk{{{\cal I}_k}} %% Native information space
\def\ifst{{{\cal I}_t}} %% Native information space
\def\imap{{\kappa}}
\def\imapndet{{\imap_{ndet}}}
\def\imapprob{{\imap_{prob}}}
\def\imapstage{{\imap_{stage}}}
\def\imapapp{{\imap_{app}}}
\def\imapmom{{\imap_{mom}}}
\def\imapgauss{{\imap_{mom}}}
\def\imapsf{{\imap_{sf}}}
\def\cifs{\ifs_c} %% Collapsed information space
\def\cist{\eta^c} %% Information space
\def\mifs{{\kappa}}
\def\imifs{{\Gamma^{-1}}}
\def\allp{{\Pi}} %% All plans
\def\allpc{{\Pi_\kappa}} %% All plans
\def\ite{{f_\ifs}} %% Information transition equation
\def\iteder{{f_\ifs}_{der}} %% Information transition equation
\def\hplan{{\cal H}} %% Information space
\def\difs{{\cal I}_\imap} %% Information space

\def\infX{{\vec{X}}}
\def\infx{{\vec{x}}}
\def\infU{{\vec{U}}}
\def\infu{{\vec{u}}}
\def\infTheta{{\vec{\Theta}}}
\def\inftheta{{\vec{\theta}}}
\def\inff{{\vec{f}}}
\def\infL{{\vec{L}}}
\def\infl{{\vec{l}}}


\def\Land{{\cal L}}

\def\ehat{\hat{e}}
\def\Ehat{\hat{E}}

\def\utility{{\cal U}}

% D^* definitions

\def\Gbest{{G_{best}}}
\def\Gcur{{G_{cur}}}
\def\Gvia{{G_{via}}}


%% This can be redef'ed later to be whatever we want for the robot
\def\A{{\cal A}}

%% Homeomorphism
\def\homeo{{ \;\cong\; }}

%%% The configuration space?
%\def\Q{{\cal Q}}

\def\choose#1#2{{(^{#1}_{#2})}}

\def\sgn{{\rm sgn}}
\def\sgnv{{\rm sgn}}

\def\pow{{\rm pow}}

\def\pdf{{p}}

%% closed chains
\def\Cclo{{{\cal C}_{clo}}}
\def\Cfea{{{\cal C}_{fea}}}


%% manip
\def\Csta{{{\cal C}_{sta}}}
\def\Cgr{{{\cal C}_{gr}}}
\def\Ctra{{{\cal C}_{tra}}}
\def\Cadm{{{\cal C}_{adm}}}
\def\Caobs{{{\cal C}^a_{obs}}}
\def\Cpobs{{{\cal C}^p_{obs}}}
\def\Capobs{{{\cal C}^{ap}_{obs}}}
\def\Xsta{{X_{sta}}}
\def\Xgr{{X_{gr}}}
\def\Xtra{{X_{tra}}}
\def\Ccon{{{\cal C}_{con}}}
\def\motcom{{\mu}}
\def\allmotcom{{\cal M}}


%%time var
\def\tva{{\tau}}
\def\tvb{{\sigma}}
\def\tvc{{\phi}}
\def\tvd{{g}}

%% multi
\def\multa{{\tau}}
\def\multb{{h}}
\def\cubesim{{\square}}

%% Conformation stuff
\def\confv{{q}}

%% General transformation
\def\gt{{h}}
\def\gti{{h^{-1}}}

%% Translation parameters
\def\xt{x_t}
\def\yt{y_t}
\def\zt{z_t}

%% Logical predicates
\def\lpred{\phi}
\def\qfpred{\phi}
\def\plpred{\alpha}
\def\quant{{\cal Q}}
\def\tarsk{\Phi}
\def\qftask{\phi}
\def\polys{{\cal F}} % Set of polynomials
\def\proot{{\beta}} % Polynomial root

%% Canny's method
\def\polyf{{\psi}}
\def\cmap{{h}}

%% C-space definitions
\def\C{{\cal C}}
\def\Cobs{{\cal C}_{obs}}
\def\Cfree{{\cal C}_{free}}
\def\CP{{P}}
\def\qinit{{q_{I}}}
\def\qgoal{{q_{G}}}
\def\qcur{{q_{cur}}}
\def\qnew{{q_{new}}}
\def\qiinit{{q^i_{I}}}
\def\qigoal{{q^i_{G}}}
\def\qoneinit{{q^1_{I}}}
\def\qonegoal{{q^1_{G}}}
\def\qminit{{q^m_{I}}}
\def\qmgoal{{q^m_{G}}}

\def\Xobs{{X_{obs}}}
\def\Xfree{{X_{free}}}
\def\Xcon{{X_{con}}}
\def\Xric{{X_{ric}}}
\def\xinit{{x_{I}}}
\def\xgoal{{x_{G}}}
\def\Xgoal{{X_{G}}}
\def\xcur{{x_{cur}}}
\def\xnew{{x_{new}}}

\def\B{{\cal B}}
\def\D{{\cal D}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\U{{\cal U}}
\def\W{{\cal W}}
\def\X{{\cal X}}

\def\Ufree{{\U_{free}}}

% Mapping for a singular simplex
\def\sing{{\sigma}}

\def\x{{ x}}
\def\u{{ u}}

\def\Uf{{\vec U}}
\def\Vf{{\vec V}}
\def\Wf{{\vec W}}
\def\Zf{{\vec Z}}

% Complexes
\def\Comp{{\cal K}}
\def\Cell{C}
\def\Simp{\Delta}

% van der Corput sequence
\def\vdc{{\nu}}
% General sequence
\def\genseq{{\alpha}}

\def\Re{{\mathbb{R}}}
\def\Com{{\mathbb{C}}}
\def\Z{{\mathbb{Z}}}
\def\S{{\mathbb{S}}}
\def\H{{\mathbb{H}}}
\def\Q{{\mathbb{Q}}}
\def\Nat{{\mathbb{N}}}
\def\RP{{\mathbb{RP}}}
\def\F{{\mathbb{F}}}
\def\T{{\mathbb{T}}}
\def\One{{\bf 1_G}}
\def\Ra{{\mathbb{A}}}
\def\Vs{{V}}

\def\Fcal{{\cal F}}

\def\q{{q}}

%% Randomized strategy
\def\urand{{w}}

\def\qq1{{q_1}}
\def\qk{{q_k}}
\def\qi{{q_i}}
\def\qkp1{{q_{k+1}}}
\def\qKp1{{q_{F}}}
\def\qKi{{q_{K+1}}}
\def\qKp1{{q_{F}}}
\def\qi{{q_{F}}}
\def\qxq1{{q_1}}

\def\uu1{{u_1}}
\def\uk{{u_k}}
\def\uK{{u_K}}
\def\ui{{u_i}}
\def\xk{{x_k}}
\def\xi{{x_i}}
\def\xkp1{{x_{k+1}}}
\def\xKp1{{x_{F}}}
\def\xKi{{x_{F}}}
\def\xq1{{x_1}}
\def\ukp1{{u_{k+1}}}
\def\thetak{{\theta_k}}

% These are backward actions
\def\bwactset{{U^{-1}}}
\def\bwact{u^{-1}}
\def\bwf{{f^{-1}}}

\def\octg{G^*}        % Optimal cost to go
\def\octc{C^*}        % Optimal cost to come 
\def\eoctg{G^*}       % expected Optimal cost to go
\def\eoctc{C^*}       % expected Optimal cost to come 
\def\woctg{G^*}       % worst-case Optimal cost to go
\def\wctg{G}       % worst-case cost to go
\def\woctc{C^*}       % worst-case Optimal cost to come 
\def\ctg{{G}}         % Cost-to-go   -- not necessarily optimal
\def\ctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\wctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\ctc{{C}}         % Cost-to-come -- not necessarily optimal
\def\ectg{\hat{G}^*}  % Estimated cost-to-go (A-star)
\def\ctgs{{g}}         % Cost-to-go for use in sampling chapter -- conflict with G
\def\exctg{G}       % expected Optimal cost to go
\def\exctgpl{G_\plan}       % expected Optimal cost to go
\def\exctc{C}       % expected Optimal cost to come 
\def\eoj{J^*}
\def\eojpl{J_\plan}
\def\qval{Q^*}
\def\aqval{\hat{Q}^*}
\def\qvalpl{Q_\plan}
\def\eectg{\hat{G}_\plan}

\def\cmean{\bar{c}}

\def\topi{{/\sim}} % Topological identification
\def\xb{{x_b}}

\def\Polys{{\cal P}}
\def\Poly{{P}}

%% 2D phase space for trajectory planning
\def\tphase{{S}}

%% Game theory
\def\Pa{{{\rm P}_1}}
\def\Pb{{{\rm P}_2}}
\def\Pc{{{\rm P}_3}}
\def\Pli{{{\rm P}_i}}
\def\Pn{{{\rm P}_n}}
\def\upperv{\overline{L}^*}
\def\lowerv{\underline{L}^*}
\def\ecost{{\bar{L}}}
\def\uppervm{\overline{\cal L}^*}
\def\lowervm{\underline{\cal L}^*}
\def\gamev{L^*}
\def\gameva{{L^*_a}}
\def\gamevb{{L^*_b}}
\def\gamevm{{\cal L}^*}

%% Plan definitions
\def\plan{\pi}
\def\fplan{\pi} %% Feedback
\def\iplan{\pi}
\def\pplan{\sigma} %% Partial plan
\def\planset{{\Pi}}
\def\fplanset{{\Pi}}

\def\argmax{\operatornamewithlimits{argmax}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\Pre{\operatorname{Pre}}
\def\Back{\operatorname{B}}
\def\SB{\operatorname{SB}}
\def\WB{\operatorname{WB}}
\def\Front{\operatorname{Front}}
\def\mymod{\operatorname{mod}}
\def\erf{\operatorname{erf}}
\def\hull{\operatorname{hull}}
\def\Front{\operatorname{Front}}
\def\atan2{\operatorname{atan2}}
\def\intfn{\operatorname{int}}
\def\dspan{\operatorname{span}}
\def\exp{\operatorname{exp}}
\def\adop{\operatorname{Ad}}
\def\clfn{\operatorname{cl}}
\def\Vor{\operatorname{Vor}}

\def\distr{{\triangle}}
\def\tdiff{{\Delta t}}
\def\lie{{\cal L}}
\def\phall{{\cal PH}}

\def\Cinfeq{{{\tilde C}^\infty}}

\def\truesp{\mbox{\sc{true }}}
\def\falsesp{\mbox{\sc{false }}}
\def\true{\mbox{\sc{true}}}
\def\false{\mbox{\sc{false}}}

\def\sccat{\mbox{\sc{cat}}}
\def\scdog{\mbox{\sc{dog}}}
\def\sctree{\mbox{\sc{tree}}}
\def\schouse{\mbox{\sc{house}}}

\def\qdot{{\dot q}}
\def\pdot{{\dot p}}
\def\qddot{{\ddot q}}
\def\qdddot{{q^{(3)}}}
\def\xdot{{\dot x}}
\def\xddot{{\ddot x}}
\def\yddot{{\ddot y}}
\def\ydot{{\dot y}}
\def\zdot{{\dot z}}
\def\xtdot{{{\dot x}_t}}
\def\ytdot{{{\dot y}_t}}
\def\thetadot{{\dot \theta}}
\def\thetaddot{{\ddot \theta}}
\def\adot{{\dot a}}
\def\bdot{{\dot b}}
\def\ceedot{{\dot c}}
\def\deedot{{\dot d}}
\def\fdot{{\dot f}}
\def\rdot{{\dot r}}
\def\sdot{{\dot s}}
\def\sddot{{\ddot s}}
\def\udot{{\dot u}}
\def\vdot{{\dot v}}
\def\wdot{{\dot w}}
\def\omegadot{{\dot \omega}}
\def\sigmadot{{\dot \omega}}
\def\phidot{{\dot \phi}}
\def\psidot{{\dot \psi}}
\def\alphadot{{\dot \alpha}}
\def\betadot{{\dot \beta}}
\def\gammadot{{\dot \gamma}}
\def\lambdadot{{\dot \lambda}}
\def\hdot{{\dot h}}
\def\gdot{{\dot g}}

\def\xtoq{{\kappa}}

\def\ustar{{u^*}}
\def\E{\operatorname{E}} %Expectation: $\E[X]$ (like \Pr)

\theoremstyle{plain}

%{\theorembodyfont{\rmfamily}\newtheorem{formulation}{Formulation}[chapter]}
%{\theorembodyfont{\rmfamily}\newtheorem{example}{Example}[chapter]}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Def}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{scenario}{Scenario}


\def\ds{\displaystyle\strut}
\def\idz{{\hspace{0.25in}}}

\def\disX{{\check X}}
\def\disx{{\check x}}
\def\disu{{\check u}}
\def\disU{{\check U}}
\def\disxgoal{{{\check x}_g}}
\def\disfplan{{\check \fplan}}
\def\disphi{{\check \phi}}

%% Dynamics
\def\force{{F}}
\def\moment{{N}}
\def\com{{p}} % Center of mass
\def\velcom{{\dot p}} % Center of mass
\def\acccom{{\ddot p}} % Center of mass
\def\mass{{m}}
\def\linmom{{D}} % Linear momentum
\def\angmom{{E}} % Angular momentum
\def\dens{{\sigma}}
\def\covfn{{\histx}} % Function for calculus of variations

\newcommand{\R}{{\mathcal R}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\qed}{\hfill $\blacksquare$ \hfill \\}


